ViDT: An Efficient and Effective Fully Transformer-based Object Detector

Transformers are transforming the landscape of computer vision, especially for recognition tasks. Detection transformers are the first fully end-to-end learning systems for object detection, while vision transformers are the first fully transformer-based architecture for image classification. In this paper, we integrate Vision and Detection Transformers (ViDT) to build an effective and efficient object detector. ViDT introduces a reconfigured attention module to extend the recent Swin Transformer to be a standalone object detector, followed by a computationally efficient transformer decoder that exploits multi-scale features and auxiliary techniques essential to boost the detection performance without much increase in computational load. Extensive evaluation results on the Microsoft COCO benchmark dataset demonstrate that ViDT obtains the best AP and latency trade-off among existing fully transformer-based object detectors, and achieves 49.2AP owing to its high scalability for large models. We will release the code and trained models at https://github.com/naver-ai/vidt

==> 2-relatedwork_previous.tex <==
\section{Related Work}
\label{sec:related_work}

A transformer is a deep model that entirely relies on the attention mechanism to capture long-range dependencies in data\,\citep{vaswani2017attention}. Recently, there have been numerous studies to investigate its adaptation to computer vision, namely (1)\,\underline{detection transformers} for object detection and (2)\,\underline{vision transformers} for image classification.

\noindent\textbf{Detection Transformers.} Attention mechanisms in transformers have gained significant attention in computer vision\,\citep{woo2018cbam, carion2020end, fan2020few, beal2020toward}. DETR\,\citep{carion2020end} is the first work to adapt the transformer architecture for object detection. The transformer architecture is connected with a typical convolutional neural network\,(CNN) backbone to transform the input feature map into a set of $[\mathtt{DET}]$ tokens. By leveraging them, DETR directly produces unique predictions for each ground-truth bounding box based on the set-based Hungarian loss with bipartite matching. In particular, DETR simplifies the detection pipeline by eliminating multiple hand-crafted components that encode prior knowledge, such as non-maximum suppression. Meanwhile, Deformable DETR\,\citep{zhu2021deformable} extends DETR with a deformable attention module, which is an efficient variant of transformer attention to exploit multi-scale feature maps. Thanks to the decoding pipeline in the neck, this DETR family can benefit even more by leveraging additional techniques, such as auxiliary decoding loss or iterative box refinement.

\noindent\textbf{Vision Transformers.} The application of transformers to computer vision have been limited to use with CNNs or replacing certain components. Yet, it has been recently witnessed that a pure transformer can applied directly to a sequence of image patches for image classification without relying on CNNs\,\citep{chen2021crossvit, yuan2021tokens}. ViT\,\citep{dosovitskiy2021image} and DeiT\,\citep{touvron2021training} is the pioneering work for vision transformers, but their architectures are not suitable to be a general-purpose backbone, due to the quadratic increase in complexity with image size, especially when requiring high-resolution images. As their follow-ups, PiT\,\citep{heo2021rethinking} and PVT\,\citep{wang2021pyramid} reduce the number of $[\mathtt{PATCH}]$ tokens\,(i.e., patch reduction) while increasing their channel dimension. Along with the patch reduction scheme, Swin Transformer\,\citep{liu2021swin} further enhances its efficiency by using local attention with shifted window partitions; the shifted window bridges the windows of the preceding layer, thus providing connections between different partitions. Hence, vision transformers are rapidly evolving for use in a wide range of vision tasks. \looseness=-1

\noindent\textbf{Integration of Vision and Detection Transformers.} The two different use of transformers have been studied extensively, but their integration has yet to be explored much. Except for the straightforward integration, YOLOS\,\citep{fang2021you} is the only work that attempts to converge vision and detection transformers; it achieves a pure sequence-to-sequence approach without additional components by adding $[\mathtt{DET}]$ tokens to image patches for the transformer input. However, as mentioned earlier, its strong reliance on the canonical ViT is detrimental to scalability and flexibility, and therefore it often performs worse than the straightforward approach, as shown in Figure \ref{fig:ap_vs_latency}. 

Our work aims to reconsider better integration of vision and detection transformers for a {fully} transformer-based object detector.
The proposed ViDT meets {high scalability} for large models, as well as {high flexibility} of using multi-scale features in conjunction with essential techniques, thereby achieving the best trade-off between accuracy and speed.


